Data Augmentation for Conversational AI

Advancements in conversational systems have revolutionized information access, surpassing the limitations of single queries. However, developing dialogue systems requires a large amount of training data, which is a challenge in low-resource domains and languages. Traditional data collection methods like crowd-sourcing are labor-intensive and time-consuming, making them ineffective in this context. Data augmentation (DA) is an affective approach to alleviate the data scarcity problem in conversational systems. This tutorial provides a comprehensive and up-to-date overview of DA approaches in the context of conversational systems. It highlights recent advances in conversation augmentation, open domain and task-oriented conversation generation, and different paradigms of evaluating these models. We also discuss current challenges and future directions in order to help researchers and practitioners to further advance the field in this area.

==> sections/works_table.tex <==
\section{List of current works}

\renewcommand{\arraystretch}{1.25}
\begin{table*}[!ht]
    \centering
    \caption{List of current works for Dialogue Augmentation}
    \begin{scriptsize}
    \begin{tabular}{l|c|c|c|c|c|c|c}
        \hline
        \textbf{Paper} &
        \textbf{Year} &
        \textbf{tr. Method} &
        \textbf{Level} &
        \textbf{Type} &
        \textbf{Challenges} &
        \textbf{Approach} &
        \textbf{Input} \\
        \hline
        
        \multicolumn{8}{c}{\textcolor{blue}{\textbf{Aug:} }\textbf{Generic Token-level \& Sentence-level Augmentation}} \\
        \hline
        MTL-QA~\cite{Bornea21MTLQA}
        & 2021-05 & --- & Sentence & & & Back-translation & \\
        \hline
        QANet~\cite{Yu18QANet}
        & 2018-08 & --- & Sentence & & & Back-translation & \\
        \hline
        DiPS~\cite{kumar2019DiPS}
        & 2019-06 & --- & Sentence & & Inducing diversity & Paraphrasing & \\
        \hline
        TreeMix~\cite{zhang2022treemix}
        & 2022-07 & ---       & Token    & & Meaningfulness, Diversity & Compositional & --- \\
        \hline
        SSMix~\cite{yoon2021ssmix}
        & 2021-08 & ---       & Token    & & Meaningfulness, Diversity & Compositional & --- \\
        \hline
        GECA~\cite{andreas2020GECA}
        & 2020-07 & ---       & Token    & & Meaningfulness, Diversity & Compositional & --- \\
        \hline
        DR-NSP~\cite{jia2016data}
        & 2016-08 & --- & Token & & Meaningfulness, Diversity & Compositional & --- \\ 
        \hline
        DA-PTM~\cite{kumar2020data}
        & 2020-12 & ---       & Token    & & Meaningfulness, Diversity & Replacement (LM) & --- \\
        \hline
        SCDA~\cite{gao2019SCDA}
        & 2019-07 & ---       & Token    & & Meaningfulness, Diversity & Replacement (LM) & --- \\
        \hline
        CA-PR~\cite{kobayashi2018CAPR}
        & 2018-06 & ---       & Token    & & Meaningfulness & Replacement (LM) & --- \\
        \hline
        Snippext~\cite{Miao20Snippext}
        & 2020-04 & ---       & Token    & & Meaningfulness & Replacement (all) & --- \\
        \hline
        EDA~\cite{wei2019eda}
        & 2019-11 & ---       & Token    & & Meaningfulness & Replacement (all) & --- \\
        \hline
        MaxLoss~\cite{Jungiewicz2019MaxLoss} 
        & 2019-03 & ---       & Token    & & Meaningfulness & Replacement (Synonym) & --- \\
        \hline
        
        \multicolumn{8}{c}{\textcolor{blue}{\textbf{Aug:} }\textbf{Dialogue Data Augmentation}} \\
        
        \hline
        CMI-GD~\cite{chen2023controllable}
        & 2023-07 & Prompting & Dialogue & Open-domain & Controllable Generation / Mixed-Initative & & \\
        \hline
        PLACES~\cite{chen2023places}
        & 2023-05 & Prompting & Dialogue & Open-domain & Multi-party conversations & & \\
        \hline
        BOTSTALK~\cite{kim2022botstalk}
        & 2022-12 & Prompting & Dialogue & Open-domain & multi-skill dialogues & & \\
        \hline
        WEAKDAP~\cite{chen2022weakly}
        & 2022-11 & Prompting & Dialogue & Open-domain & --- & & \\
        
        
        
        \hline
        DialAug~\cite{poddar2022dialaug}
        & 2022-10 & Generative  & Dialogue & Open-domain  & Diversity &  &  \\ 
        \hline
        CAPT~\cite{Ou22CAPT}
        & 2022-10 & Generative  & Dialogue & Open-domain  & Diversity & Counterfactual & H, CQ, CA \\ 
        \hline
        DlDistill~\cite{zhang2020DlDistill}
        & 2020-11 & Both Ret. \& Gen. & Dialogue & Open-domain & Diversity & Unpair data & --- \\
        \hline
        CVAE-GAN~\cite{Li2019CVAEGAN}
        & 2019-01 & Generative & Dialogue & Open-domain & Diversity & Generative model & H, CQ, CA \\      
        \hline
        CUDA-DST~\cite{lai2022CUDADST}
        & 2022-09 & Generative & Dialogue & Task-oriented & Generalization, Diversity & User Dialogue Act (UDA) & H \\
        \hline
        COCO~\cite{Li2021coco}
        & 2021-03 & Retrieval & Dialogue & Task-oriented & Generalization, Diversity & UDA, Counterfactual & H \\
        \hline
        PARG~\cite{gao2020PARG}  
        & 2020-07 & Generative & Dialogue & Task-oriented
        & Diversity & Paraphrasing & H, CA \\
        \hline
        RDA~\cite{Yin2020RDA} 
        & 2020-04 & Generative & Dialogue & Task-oriented & Quantity, Diversity & RL-based   & P, CQ, CA \\    
        \hline

    \end{tabular}
    \end{scriptsize}	
    \label{table:aug_papers}
\end{table*}

\renewcommand{\arraystretch}{1.25}
\begin{table*}[!ht]
    \centering
    \caption{List of current works for Dialogue Generation: Open-Domain}
    \begin{scriptsize}
    \begin{tabular}{l|c|c|c|c|c|c|c}
        \hline
        \textbf{Paper} &
        \textbf{Year} &
        \textbf{tr. Method} &
        \textbf{Level} &
        \textbf{Type} &
        \textbf{Challenges} &
        \textbf{Approach} &
        \textbf{Input} \\
        \hline
        
        \multicolumn{8}{c}{\textcolor{blue}{\textbf{ODD Gen:} }\textbf{Single-turn generation}} \\
        \hline
        GRADA~\cite{maharana2022grada}
        & 2022-10 & \tiny \specialcell{{Generative,}\\{Augmentation}}
        & QA pair & Open-domain & \tiny Informative, Diverse & 2, 3, 4    & KG \\
        \hline
        G-DAUG~\cite{Yang2020DAug}
        & 2020-11 & Generative & QA pair & --- & & 2, 3, 4    & --- \\
        \hline
        PAQ~\cite{lewis2021paq}
        & 2021    & Hybrid-GR  & QA pair & Open-domain & & 1, 2, 3, 4 & KB \\
        \hline
        TQA-SD~\cite{puri2020training}
        & 2020-02 & Generative & QA pair & --- & & 2, 3, 4    & --- \\
        \hline
        Alberti19~\cite{alberti2019synthetic}
        & 2019-07 & Generative & QA pair & --- & & 2, 3, 4    & P \\
        \hline
        % Lewis19~\cite{lewis2019unsupervised}
        % & 2019-07 & Generative & QA pair & --- & & 2, 3, 4    & P \\
        % \hline

        \multicolumn{8}{c}{\textcolor{blue}{\textbf{ODD Gen:} }\textbf{Multi-turn generation}} \\
        \hline
        % Baize~\cite{Xu2023Baize}
        % & 2023-04 & Prompting & Dialogue & Open-domain & & & \\
        % \hline
        SODA~\cite{kim2022simseek}
        & 2023-05 & prompting & Dialogue & Open-domain &
        --- & 2, 3, 4   & KG \\
        \hline
        RSODD~\cite{kim2022simseek}
        & 2022-07 & prompting & Dialogue & Open-domain &
        Human-AI collaborative & 2, 3, 4   & H, B, P \\
        \hline
        
        SIMSEEK~\cite{kim2022simseek}
        & 2022-12 & Generative & Dialogue & Open-domain &
        \tiny \specialcell{{Blinded to the answer-containing passage,} 
        \\ {rely on background information B}} & 2, 3, 4   & H, B, P \\
        \hline
        % GCN~\cite{lin2022GCN}
        % & 2022-09 & Hybrid-GR, RL & Dialogue & Open-domain & Real scenarios & 1, 2, 3, 4 & \\
        % \hline      
        DG2~\cite{wu2022dg2}
        & 2022-09 & Generative & Dialogue & Open-domain &
        \tiny Consistency, Sub passage selection & 1, 2, 3, 4 & P, H \\
        \hline
        MultiCQAG~\cite{hwang2022multiCQG}
        & 2022-11 & Generative & Dialogue & Open-domain &
        \tiny Consistency, Question Types & 1, 2, 3, 4 & H, P \\
        \hline
        CQAG-AR~\cite{hwang2022CQAGAR}
        & 2022-10 & Generative & Dialogue & Open-domain &
        \tiny Consistency, Answer revision & 2, 3, 4    & H, P \\
        \hline
        CoHS-CQG~\cite{do2022cohsCQG}
        & 2022-10 & Generative & Dialogue & Open-domain &
        \tiny Consistency, Sub Passage/History selection & 1, 2, 3, 4 & H, P \\
        \hline
        ChainCQG~\cite{gu2021chaincqg}
        & 2021-04 & Generative & Dialogue & Open-domain &
        \tiny Consistency & 1, 2, 3, 4 & H \\
        \hline
        % SHSF~\cite{Qi2020SHSF}
        % & 2020-11 & ---        & ---      & Open-domain & & ---        & --- \\
        % \hline
        AU-CQG~\cite{nakanishi2019AUCQG}
        & 2019-11 & Hybrid-GR & Dialogue & Open-domain &
        \tiny Consistency, Sub passage selection & 1, 3, 4 & H, P \\
        % \hline
        % ReDR~\cite{pan2019ReDR}
        % & 2019-07 & Generative & Dialogue & Open-domain &
        % \tiny Consistency, Coreference alignment & 2, 3 & H \\
        \hline
        CFNet~\cite{gao2019CFnet}
        & 2019-07 & Generative & Dialogue & Open-domain &
        \tiny Consistency, Coreference alignment & 1, 3, 4 & H, P \\
        \hline

        \multicolumn{8}{c}{\textcolor{blue}{\textbf{ODD Gen:} }\textbf{Target-oriented dialogue systems}} \\
        % \hline
        % I-Pro~\cite{Lei2022IPro}
        % & 2022-07 & Retrieval & Dialogue & Target-oriented &
        % \tiny \specialcell{{Consistency, Target achievement,} \\ {User satisfaction}}
        % & 1, 2, 3 & H, Ext. KG, G \\
        \hline
        COLOR~\cite{Wang2023COLOR}
        & 2023-05 & Generative & Dialogue & Target-oriented &
        \tiny Consistency, target achievement & 1, 2, 3 & H, Ext.KG, G \\
        \hline
        HiTKG~\cite{ni2022hitkg}
        & 2022-10 & Generative & Dialogue & Target-oriented &
        \tiny Consistency, target achievement & 1, 2, 3 & H, Ext.KG, G \\
        \hline
        EGRL~\cite{Xu20EGRL}
        & 2021-01 & Generative & Dialogue & Target-oriented &
        \tiny Consistency, target achievement & 1, 2, 3 & H, Ext.KG, G \\
        \hline
        KnowHRL~\cite{Xu20KnowHRL}
        & 2020-04 & Generative & Dialogue & Target-oriented &
        \tiny Consistency, target achievement & 1, 2, 3 & H, Ext.KG, G \\
        
        \hline
        TopKG~\cite{yang2022topkg}
        & 2022-10 & Generative & Dialogue & Target-oriented &
        \tiny Consistency, target achievement & 1, 2, 3 & H, Ext.KG, G \\
        \hline
        CKC~\cite{Zhong2021CKC}
        & 2021-12 & Generative & Dialogue & Target-oriented &
        \tiny Consistency, target achievement & 1, 2, 3 & H, Ext.KG, G \\
        \hline
        DKRN~\cite{Qin2020DKRN}
        & 2020-06 & Retrieval  & Dialogue & Target-oriented &
        \tiny Consistency, target achievement & 1, 2, 3 & H, Int.KG, G \\
        \hline
        TGODC~\cite{tang2019target}
        & 2019-07 & Retrieval & Dialogue & Target-oriented &
        \tiny Consistency, target achievement & 1, 2, 3 & H, Int.KG, G \\
        \hline
        TGCP~\cite{kishinami2022TGCP}
        & 2022-10 & & 1-turn Dialogue & Target-oriented & & & \\
        \hline
        CRG~\cite{gupta2022CRG}
        & 2022-07 & & 1-turn Dialogue & Target-oriented & & & \\
        \hline
        OTTers~\cite{sevegnani2021otters}
        & 2021-08 & & 1-turn Dialogue & Target-oriented & & & \\
        \hline
        % KPN~\cite{Zhu2021KPN}
        % & 2021-07 & & 1-turn Dialogue & Target-oriented & & & \\
        % \hline
        % DuConv~\cite{wu2019DuConv}
        % & 2019-07 & Both G\&R  & Dialogue & Target-oriented &
        % \tiny Consistency, target achievement & 2       & H, Ext.KG, G \\
        % \hline   
        % SKT/ST-KG~\cite{zhan2021SKTKG}
        % & 2021-06 & Generative & Dialogue & Open-domain &
        % \tiny Consistency (knowledge transition) & 1 &  \\
        % \hline
    \end{tabular}
    \end{scriptsize}	
    \label{table:ODD_papers}
\end{table*}       

\renewcommand{\arraystretch}{1.25}
\begin{table*}[!ht]
    \centering
    \caption{List of current works for Dialogue Generation: Task-oriented}
    \begin{scriptsize}
    \begin{tabular}{l|c|c|c|c|c|c|c}
        \hline
        \textbf{Paper} &
        \textbf{Year} &
        \textbf{tr. Method} &
        \textbf{Level} &
        \textbf{Type} &
        \textbf{Challenges} &
        \textbf{Approach} &
        \textbf{Input} \\
        \hline

        \multicolumn{8}{c}{\textcolor{blue}{\textbf{ToD Gen:} }\textbf{Schema-guided generation}} \\
        \hline
        SGD~\cite{Rastogi2020SGD}
        & 2020-06 & Generative & Dialogue & Task-oriented & Task completion & --- & --- \\
        \hline
        M2M~\cite{Shah2018M2M}
        & 2018-01 & Generative & Dialogue & Task-oriented & Task completion & --- & --- \\
        \hline
        
        \multicolumn{8}{c}{\textcolor{blue}{\textbf{ToD Gen:} }\textbf{Simulator-Agent Interaction}} \\
        \hline
        ICL-US~\cite{Terragni2023ICLUS}
        & 2023-06 & In-Context & Dialogue & Task-oriented & Task completion, Diversity & --- & --- \\
        \hline
        Unified-US~\cite{wan2022unified}
        & 2022-12 & Generative & Dialogue & Task-oriented & Task completion & --- & --- \\
        \hline
        SimulatedChat~\cite{mohapatra2021simulatedchats}
        & 2021-11 & Hybrid-GR & Dialogue & Task-oriented & Task completion & --- & --- \\
        \hline
        JOUST~\cite{tseng2021DSUSRL}
        & 2021-08 & Generative & Dialogue & Task-oriented & Task completion & --- & --- \\
        \hline
        TUS~\cite{lin2021TUS}
        & 2021-07 & Generative & Dialogue & Task-oriented & Task completion & --- & --- \\
        \hline
        LaRL~\cite{zhao2019LaRL}
        & 2019-06 & Generative & Dialogue & Task-oriented & Task completion & --- & --- \\
        \hline
        
        \multicolumn{8}{c}{\textcolor{blue}{\textbf{ToD Gen:} }\textbf{E2E dataset creation}} \\
        \hline
        DIALOGIC~\cite{li2022DIALOGIC}
        & 2022-12 & In-context & Dialogue & Task-oriented & Controllable Gen. & & \\
        \hline
        LAD~\cite{mehri2022lad}
        & 2022-09 & Prompting  & Dialogue & Task-oriented & ZSH. Generalisation, Diversity & & \\
        \hline
        NeuralWOZ~\cite{kim2021neuralwoz}
        & 2021-08 & Retrieval & Dialogue & Task-oriented & Task completion, Unseen domain & --- & --- \\
        \hline
        VHDA~\cite{yoo2020VHDA}
        & 2020-11 & Generative & Dialogue & Task-oriented & Task completion & --- & --- \\
        \hline
    
    \end{tabular}
    \end{scriptsize}	
    \label{table:TOD_papers}
\end{table*}


